SurfelGAN: Synthesizing Realistic Sensor Data for Autonomous Driving

Autonomous driving system development is critically dependent on the ability to replay complex and diverse traffic scenarios in simulation. In such scenarios, the ability to accurately simulate the vehicle sensors such as cameras, lidar or radar is essential. However, current sensor simulators leverage gaming engines such as Unreal or Unity, requiring manual creation of environments, objects and material properties. Such approaches have limited scalability and fail to produce realistic approximations of camera, lidar, and radar data without significant additional work. In this paper, we present a simple yet effective approach to generate realistic scenario sensor data, based only on a limited amount of lidar and camera data collected by an autonomous vehicle. Our approach uses texture-mapped surfels to efficiently reconstruct the scene from an initial vehicle pass or set of passes, preserving rich information about object 3D geometry and appearance, as well as the scene conditions. We then leverage a SurfelGAN network to reconstruct realistic camera images for novel positions and orientations of the self-driving vehicle and moving objects in the scene. We demonstrate our approach on the Waymo Open Dataset and show that it can synthesize realistic camera data for simulated scenarios. We also create a novel dataset that contains cases in which two self-driving vehicles observe the same scene at the same time. We use this dataset to provide additional evaluation and demonstrate the usefulness of our SurfelGAN model.

==> 03_overview.tex <==
\section{Overview}
\label{Section:Overview}
The rest of this paper is organized as follows: In the Approach section, we will describe the two core components of our system, namely, scene reconstruction module and image synthesis module. Both components are crucial for obtaining best results. In the Experimental Results section, we will first describe the dataset we are using, then discuss our evaluation metrics and show our experimental results.

==> Figure/surfel.tex <==

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Figure/data/surfel.png}
\caption{Left: Texture mapped surfel for which we create virtual grids on each surfel disk to enhance the level of representability. Right: Camera image, rendered RGB~image, the semantic image, and the instance image (from top to bottom). }
\label{fig:surfel}
\end{figure}

==> Table/breakdown.tex <==

\begin{table}[!tbp]
  \footnotesize
  \centering
  \begin{tabular}{lcccc}
  \toprule
  Perturbation & mAP@.5 & mAP@.75 & mAP\\
  \hline
   Small & 0.574 & 0.174 & 0.257\\
   Median  & 0.547 & 0.173 & 0.246\\
   Large  & 0.488 & 0.153 & 0.218\\
  \bottomrule
  \end{tabular}
 \caption{Detector metric break down at different perturbation level on WOD-EVAL-NV}
 \label{tab:breakdown}
\end{table}

==> Table/detector.tex <==
\begin{table}

  \footnotesize
  \centering
  \begin{tabular}{|l|c|c|c|c|}
  \toprule
  \hline
  Training Set & mAP@.5 & mAP@.75 & mAP & mAR\\
  \hline
   WOD(train) & 0.219 & 0.108 & 0.119 & \textbf{0.190}\\
   WOD(train) + Surfel Image & 0.228 & 0.111 & 0.120 & 0.180\\
   WOD(train) + GAN Image & \textbf{0.254} & \textbf{0.121} & \textbf{0.130} & 0.183\\

  \hline
  \bottomrule
  \end{tabular}
{%
 \caption{Detector metric on Open Dataset validation set when trained with different combination of data.}
 \label{tab:baseline-comparison}
}

\end{table}



==> Table/quantitative.tex <==
\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{l|cccc|cccc|cccc|c}
\toprule
  & \multicolumn{4}{c|}{WOD-TRAIN-NV} & \multicolumn{4}{c|}{WOD-EVAL} & \multicolumn{4}{c|}{WOD-EVAL-NV} & MV \\
  
  & AP@50 $\uparrow$ & AP@75 $\uparrow$ & mAP $\uparrow$ & mAR $\uparrow$ & AP@50 & AP@75 & mAP & mAR & AP@50 & AP@75 & mAP & mAR & L1 $\downarrow$\\
\midrule  
Surfel & 0.444 & 0.168 & 0.211 & 0.342 & 0.521 & 0.168 & 0.239 & 0.371 & 0.462 & 0.154 & 0.213 &0.348 & 0.262 \\
  
Ours (S) & 0.508 & 0.177 & 0.236 & 0.359 & 0.576 & 0.164  &0.252 & 0.341 & 0.514 & 0.159 & 0.230 & 0.358 &\textbf{0.229} \\
   
Ours (SA) & 0.554 & 0.200 & 0.259 & 0.382 & 0.610 & 0.174 & 0.266 & 0.394 & 0.567 & 0.180 & 0.257 & 0.387 & 0.240 \\

Ours (SAC) & \textbf{0.564} & \textbf{0.200} & \textbf{ 0.263 } & \textbf{0.385} & \textbf{0.620} & \textbf{0.181} & \textbf{0.272} &\textbf{0.400} & \textbf{0.570} & \textbf{0.181} & \textbf{0.258} & \textbf{0.388} & 0.238 \\

Real & - & - & - & - & 0.619 & 0.198 & 0.281& 0.424 & - & - & - & - & -\\

\bottomrule
  \end{tabular}
\caption{Quantitative comparision between our method and baselines on 4 datasets. WOD-TRAIN-NV/WOD-EVAL-NV: novel view dataset created on Waymo Open Dataset Trainin and Evaluation split respectively. WOD-EVAL: Waymo Open Dataset Evaluation split. DC: Dual-Camera-Pose Dataset. Surfel-I: our texture enhanced surfel image. L1: only use l1 reconstruction loss. P: use l1 loss + GAN loss with paired training data, P+NP: use both paired and unpaired training data. Real: real images. These are only available for WOD-EVAL and MV. }
\label{tab:baseline-comparison}
\end{table*}


